Attention Actor-Critic algorithm for Multi-Agent Constrained Co-operative Reinforcement Learning

In this work, we consider the problem of computing optimal actions for Reinforcement Learning (RL) agents in a co-operative setting, where the objective is to optimize a common goal. However, in many real-life applications, in addition to optimizing the goal, the agents are required to satisfy certain constraints specified on their actions. Under this setting, the objective of the agents is to not only learn the actions that optimize the common objective but also meet the specified constraints. In recent times, the Actor-Critic algorithm with an attention mechanism has been successfully applied to obtain optimal actions for RL agents in multi-agent environments. In this work, we extend this algorithm to the constrained multi-agent RL setting. The idea here is that optimizing the common goal and satisfying the constraints may require different modes of attention. By incorporating different attention modes, the agents can select useful information required for optimizing the objective and satisfying the constraints separately, thereby yielding better actions. Through experiments on benchmark multi-agent environments, we show the effectiveness of our proposed algorithm.

==> BroaderImpact.tex <==
\section{Broader Impact}
\label{sbi}
We have considered a constrained RL setting where the agents need to learn optimal actions that satisfy the constraints on their actions from only the state and cost samples (model-free setting). As discussed in the Introduction section, our algorithm can be deployed in a warehouse setting where a group of robots are deployed to move objects from source to desired destinations. We can specify the collision constraints among the robots such that the average number of collisions between the robots can be maintained at the desired level. 

However, our algorithm, in the current form, is not suitable for critical applications like medical purposes. If the distribution of samples received during the training varies even slightly from the distribution during deployment, the mean penalty achieved by the RL algorithm may not be less than the prescribed penalty threshold. This might be manageable in non-critical applications, but not favorable in critical applications. 
